Blockaid: Data Access Policy Enforcement for Web Applications

Modern web applications serve large amounts of sensitive user data, access to which is typically governed by data-access policies. Enforcing such policies is crucial to preventing improper data access, and prior work has proposed many enforcement mechanisms. However, these prior methods either alter application semantics or require adopting a new programming model; the former can result in unexpected application behavior, while the latter cannot be used with existing web frameworks. Blockaid is an access-policy enforcement system that preserves application semantics and is compatible with existing web frameworks. It intercepts database queries from the application, attempts to verify that each query is policy-compliant, and blocks queries that are not. It verifies policy compliance using SMT solvers and generalizes and caches previous compliance decisions for better performance. We show that Blockaid supports existing web applications while requiring minimal code changes and adding only modest overheads.

==> future.tex <==
\name is a privacy enforcement system that supports legacy web applications and
incurs low overhead.
While we have demonstrated the feasibility of our approach,
here we outline two future directions.

\paragraph{Specialized decision procedures.}
While SMT solvers are flexible and versatile,
they 
% SMT solvers, albeit flexible and versatile,
may not be the most performant tool for verifying query compliance.
One alternative is the chase procedure~\cite{aho79:joins,maier79:chase},
which has been used to study query determinacy~\cite{Gogacz15,nash07:det}
and can be naturally extended to compliance.
We hypothesize that for the class of views and queries encountered in the
privacy use case, compliance holds exactly when the chase terminates
in a small number of rounds.
We defer refining and proving this hypothesis, as well as experimenting with
various chase implementations~\cite{benedikt17:chase}, to future work.

\paragraph{Checking updates.}
We plan to extend \name to verify privacy compliance for database updates.
We envision this extension taking two steps.
First, we check updates against separate ``update'' policies, which can
differ from the ``read'' policies as 
as some information should be accessible but not modifiable.
We expect the update policies to be much easier to specify and check,
since SQL \texttt{INSERT INTO}, \texttt{UPDATE}, and \texttt{DELETE} statements
are simpler than \texttt{SELECT}.
Second, we ensure that the updates maintain schema constraints,
which are assumed to hold by \name's checking of \texttt{SELECT}.
Some constraints (like primary keys) are maintained automatically by the database, while others we have to check in \name.

% \paragraph{Policy synthesis.}
% To use \name on an existing application, a developer must specify a privacy
% policy for the application as view definitions, a manual undertaking that
% might hinder \name's adoption.
% To alleviate this burden, we plan to study \emph{automatic synthesis} of
% privacy policies by observing queries issued by the application.
% The synthesized policy can then be reviewed by a human and put into production.


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

